One Network Fits All? Modular versus Monolithic Task Formulations in Neural Networks

Can deep learning solve multiple tasks simultaneously, even when they are unrelated and very different? We investigate how the representations of the underlying tasks affect the ability of a single neural network to learn them jointly. We present theoretical and empirical findings that a single neural network is capable of simultaneously learning multiple tasks from a combined data set, for a variety of methods for representing tasks -- for example, when the distinct tasks are encoded by well-separated clusters or decision trees over certain task-code attributes. More concretely, we present a novel analysis that shows that families of simple programming-like constructs for the codes encoding the tasks are learnable by two-layer neural networks with standard training. We study more generally how the complexity of learning such combined tasks grows with the complexity of the task codes; we find that combining many tasks may incur a sample complexity penalty, even though the individual tasks are easy to learn. We provide empirical support for the usefulness of the learning bounds by training networks on clusters, decision trees, and SQL-style aggregation.

==> old_text.tex <==
\section{Old text}

\subsubsection{Exponential dependency on depth is necessary -- Data is Non-trivial to Separate into Individual Tasks}\label{sec:case1}

We consider the case when the data for the different tasks is non-trivial to separate out. We first show that there exist certain settings in this case where a single learner provably needs a significantly higher time or sample complexity to learn multiple tasks, than what is required to solve each individual task. Based on the theoretical result, we construct a synthetic task where a single learner for multiple tasks needs a much larger number of samples than a separate learner for every task. We then relax the synthetic setting, and show that a single network does significantly better if the data from the different tasks becomes easier to separate out.
%\subsection{Theoretical analysis}

We describe a setting where using a single network is provably bad. The data points are $b+d$ dimensional binary vectors. The label of any data point is the XOR ($\oplus$) of some unknown parity function computed on the first $b$ bits and a simple function computed on the last $d$ bits (any easy to learn function suffices, for e.g. a function which only depends on the last bit), along with some noise.
 
%\begin{quote}
 %   Label = (unknown noisy parity computed on the first $b$ bits) \\
%\hspace{5pt}XOR  (some simple function of the next $d$ bits)
%\end{quote}

Formally, for any $b+d$ dimensional datapoint $x$, let $x[:b]$ denote the first $b$ bits of $x$, and let $x[b:]$ denote the last $d$ bits. Let $v\in \{0,1\}^b$. Let $e$ be a Bernoulli random variable which is 1 with probability 0.1. The labelling function $f$ is a function from $\{0,1\}^{b+d} \rightarrow \{0,1\}$, defined as follows,
\begin{align*}
f(x) = ((\langle v,x[:b]\rangle \mod 2) \oplus e) \oplus (\text{any simple function computed on } x[b:]).
\end{align*}

Note that learning $f$ is also a multi-task learning problem where the individual tasks are easy. The reason for this is as follows. Suppose we have multiple tasks with a separate simple classification function for every task, with the function being determined by a parity computed on the first $b$ bits. Then solving the multi-task learning problem is equivalent to learning $f$. Note that learning each individual task here is easy as it only requires learning the simple function.

We show hardness of learning $f$ using any  neural network whose architecture is symmetric to the coordinates of the input and hence is invariant to the ordering of the coordinates. We consider such symmetric architectures as they represent a vanilla, giant network instead of a more modular network. Note that almost all commonly used neural networks architectures treat all coordinates of the input symmetrically and hence Theorem \ref{thm:parity} applies to them.  The proof relies on the hardness of learning \emph{parity with noise}, the definition of the problem and the proof overview appears in the appendix.

\begin{restatable}{thm}{parity}\label{thm:parity}
Conditioned on the hardness of the parity with noise problem, any model which treats all coordinates symmetrically---and hence is invariant to a permutation applied to the coordinates of all the data points---needs at least $\Omega(d^b)$ time or samples to learn $f$. Hence a vanilla neural network which is invariant to a permutation of the coordinates needs at least $\Omega(d^b)$ time or samples to learn $f$. In contrast, learning a separate model for every set of the first $b$ bits needs $O(2^b)$ samples.
\end{restatable}


\subsection{Main Results and Overview}

We now summarize our setup and results and give an overview of the paper. We show that a key property which determines learnability of multiple tasks is the degree of separation of the data points from the different tasks. To demonstrate this, we consider two different scenarios for multi-task learning and examine them theoretically and empirically. 

\begin{tightenumerate}

\item \emph{Data is non-trivial to separate into individual tasks (Section \ref{sec:case1}):} The first scenario we consider is when the  data-points from the different tasks are non-trivial to separate out. This would be the case if the data distributions for the different tasks are close to each other.

\item \emph{Data is naturally clustered into individual tasks (Section \ref{sec:case2})}: The second scenario is when the data distributions for the different tasks are well-separated. In this case, doing any simple clustering (such as a $k$-means clustering) on the combined data would cluster the data based on the task.

\end{tightenumerate}


Theorem \ref{thm:parity} shows that learning multiple tasks using a single neural network can be provably hard in the first case---even though the individual tasks are easy to learn. Motivated by the theoretical result, in Section \ref{sec:case1exp} we construct a synthetic setting which empirically demonstrates that learning multiple tasks with a single neural network can be hard when the different tasks are difficult to separate out. By systematically varying the degree of separation of the different tasks in the synthetic setting, we also show that making the different tasks easier to separate significantly helps a single neural network to learn them. We investigate this further in Section \ref{sec:case2} and empirically show that when the data from the different tasks is well-separated into distinct clusters, a single neural network can simultaneously do well on all of them. Theorem \ref{thm:mult} provides theoretical evidence for this ability of neural networks to learn multiple well-separated tasks, using the recent framework of \citet{arora2019fine}.

		

\subsection{Learnability when Data is Naturally Clustered into Separate Sub-tasks}

\mult*
\noindent \emph{Proof sketch: }
\citet{arora2019fine} show that if the following Gram matrix corresponding to the ReLU activation function is well-behaved, then the function is learnable with gradient descent. Let $\{x_i\in [n]\}$ be the training set. The matrix $H^{\infty} \in \mathbb{R}^{n \times n}$ is defined as follows.

\begin{align*}
H_{ij}^{\infty} = \frac{x_i^T x_j(\pi- \arccos{(x_i^T x_j)})}{2\pi},\; \forall\; i,j \in [n].
\end{align*} 

Informally, \citet{du2018gradient} show that the gradient descent on a two layer ReLU network converges to small error as long as the minimum eigenvalue of the matrix $H^{\infty}$ is bounded from below. \citet{arora2019fine} additionally bound the generalization error, and show that for any 1-Lipchitz loss function the generalization error of the two layer ReLU network found by gradient descent is at most 
\begin{align*}
    \sqrt{\frac{y^T(H^{\infty})^{-1}y}{n}}.
\end{align*}

Here $y$ is the vector of the labels. Therefore, if $y^T(H^{\infty})^{-1}y$ is a constant for a task, then the generalization error decreases at a $\sqrt{1/n}$ rate.

Note that if the data points for the individual tasks are orthogonal, then the cross-terms in the matrix $H^{\infty}$ are 0 and hence $y^T(H^{\infty})^{-1}y$ for the overall problem is just the sum of the contributions from each of the tasks. Hence the overall problem can be learned with sample complexity equal to the sum of the sample complexity of learning each individual task.

If the data points for the tasks are close to being orthogonal, then we can use matrix perturbation bounds to control the error and show that the property is still approximately satisfied (currently ongoing work).	\hfill \qed

\subsection{Additional Experiments for Section \ref{sec:case2}}\label{sec:lin}

\paragraph{Linear classifier for each task:} In this experiment, the data is drawn from $k$ clusters, and from a mixture of two well-separated Gaussians in each cluster. Data points from the two Gaussians within each cluster are assigned two different labels, for $2k$ labels in total. Fig. \ref{fig:lin1} below shows an instance of this task in two dimensions, the red circles represent the clusters, and there are two classes drawn from well-separated Gaussians from each cluster. In high dimensions, the clusters are very well-separated, and doing a $k$-means clustering to identify the $k$ cluster centers and then learning a simple linear classifier within each cluster gets near perfect classification accuracy.  Fig. \ref{fig:lin2} shows the performance of a single neural network trained on this task. We can see that a single neural network still gets good performance with a modest increase in the required number of samples.

\begin{figure}
\centering
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{cluster_lin.png}
    \caption{An instance of the problem with multiple clusters, each cluster is indicated by a red circle.}
    \label{fig:lin1}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
    \centering
    \includegraphics[width=\textwidth]{cluster_lin_plot.png}
    \caption{Test accuracy vs. number of points per cluster}
    \label{fig:lin2}
\end{subfigure}
\label{fig:lin}
\caption{Experiment where data is clustered into tasks. A single neural network does well even when there are multiple clusters.}
\end{figure}

\subsection{Additional Experiments for Section \ref{sec:case1}}

\begin{figure}
\centering
    \includegraphics[width=0.45\textwidth]{label_onehot.png}
    \caption{Test accuracy vs. number of points per context (task) when the task label is encoded in one-hot representation and hence the tasks are easier to separate.}
    \label{fig:one_hot}
\end{figure}

\subsection{Related applied work}\label{sec:related}

The success of neural networks at multi-task learning has also been demonstrated in more applied work. Here, we outline a few examples:

\begin{tightenumerate}
    \item 	In natural language processing, \citet{tsai2019small} show that a single model can solve machine translation across more than 50 languages. As reflected in many other works as well \citep{johnson2017google,aharoni2019massively,bapna2019massively, devlin2018bert}, a trend in NLP seems to be to use one model for multiple languages, and even multiple tasks.
	\item Success has also been achieved in training a multiple model across tasks in very different domains, such as speech and language \cite{kaiser2017one}.
	\item There is also work on training extremely large neural networks which have the capacity to learn multiple tasks \cite{shazeer2017outrageously}.
	\end{tightenumerate}
	
	
	%%%%%% intro
	
	We note that the learning of such combined functions could have been engineered by hand:
%\aga{representations+decoders, right?}: 
there exist 
efficient algorithms for learning clusterings or such decision trees, and it
is easy to learn the linear functions given the partitioned 
data. Likewise, these classes of functions are all known to be learnable by other 
methods, given an appropriate transformation of the input features. The key point is 
that {\em the two-layer neural network can jointly learn
the task coding scheme and the task-specific function without special 
engineering of the architecture}. That is, it is unnecessary to engineer a way 
of partitioning of the data into separate tasks prior to learning.
Relatedly, since this is feasible, the time and sample requirements of learning multiple tasks on a single network in general is insufficient to explain the modularity observed in biological neural  networks---i.e., we cannot explain the presence of modularity from such general considerations. 
%\aga{Way too bold a claim. For example,
%convolutional structure is essential for vision - so visual cortex being separate from, say, motor cortex could be
%argued to be driven by fundamental requirements of learning. Also more generally in neuroscience, requirements
%of learning are always int he context of some resource limitation - energy, neurons, etc.}.


All our theoretical results are based upon a fundamental theorem that shows that analytic functions can be efficiently learnt 
by wide two-layer neural networks with standard activation functions (such
as ReLU), using stochastic gradient descent from a random initialization. Specifically, for very wide networks, we derive novel generalization bounds for multivariate analytic functions (see Theorem~\ref{thm:multivar}) by relating wide networks to
kernel learning with a specific network-induced kernel \cite{jacot_neural_2018,du_gradient_2019,allen-zhu_learning_2019,arora_finegrained_2019,lee_wide_2019}, known as 
the  \emph{neural tangent kernel} (NTK) \cite{jacot_neural_2018}. We further develop a \emph{calculus of bounds}
showing that the sum, product, ratio and composition of analytic functions is also learnable, with bounds constructed using 
the familiar product and chain rules of
univariate calculus (Corollaries \ref{cor:prod_rule}, 
\ref{cor:chain_rule}).  These above learnability results may be of independent interest; for 
example, they can be used to show that natural physical laws like the gravitational force equations can be efficiently learnt 
by neural networks (see Section~\ref{sec:learning_gravity}). 
(\textcolor{red}{ADD A REFERENCE TO THE THEOREM IN SUPPLEMENTARY MATERIAL})


We then show that Theorem~\ref{thm:multivar} can be used to establish the learnability of not only analytic
functions, but also functions of a combinatorial nature, which can represent our task coding schemes.  
%As a secondary contribution of the work, these
%families of task codes provide a broad family of functions that we prove are
%learnable by depth-two neural networks with standard activation functions %(such
%as ReLU), using stochastic gradient descent from a random initialization. 
In particular, we find that shallow decision trees using either Boolean or linear 
decision nodes (with an adequate margin) are learnable (see Theorem \ref{thm:decisiontree_informal} and \ref{thm:decisiontreemargin_informal}). 
We show furthermore
that SQL-style aggregation queries over a fixed database, written as a functions of 
the parameters of the query, can also be learned this way; and that in general, programs built by the composition of a small
number of such
learnable functions are also learnable.

Our key contribution is that we show these functions are efficiently learned by SGD. Indeed, although universal approximation
theorems show that such functions can be represented by (sufficiently wide) two-layer neural networks,
some expressible functions are believed not to be learnable
\cite{klivans2009cryptographic}. We supplement the theoretical bounds with experiments showing that
such functions are indeed learned in practice.

%%%% conclustion

\section{Future Work}
[[Xin: This should be expanded.]] 

1. Note although we showed neural networks can learn programs of the aforementioned classes, sub-programs are not reused in the current learning framework. This may be limited by the two layer structure of the neural network.

2. Going from vector input and vector output to object input/output.

3. Modules are not physically separated, i.e. they are learned in the same network, but can still be logically separated using different subspaces. 

\section{Conclusion}

Our results indicate that a single neural network could have the ability to learn tasks across multiple, diverse domains. However, having a modular architecture still has other benefits:

\begin{tightenumerate}
 \item   \emph{Energy consumption and computational efficiency:} Modular learners  use less energy and computation, as only a subpart of the entire model needs to evaluate any data point.
\item	\emph{Interpretability:} Modular architectures can be more interpretable, as it is clearer what role each part of the model is performing.% We note that when we combine modules into a network they are not physically separated but can still be logically separated as their outputs reside in different subspaces. %Further a modular program reuses sub-programs are not reused in the current learning framework. This may be limited by the two layer structure of the neural network.

	
\end{tightenumerate}	

It would be very interesting if some of these benefits of modularity could be extended to a single model as well. For instance, is it necessary for a giant, non-modular network to have sub-parts which perform simple computations, and which can be extracted from the larger network? This could help in interpreting and understanding large neural networks. 

Though we primarily focused on two-layer neural networks with ReLU activations, an open question is what models
are optimal for different tasks and task combinations. For example, our results are applicable
even for learning using kernel methods since a two-layer infinite width network can be 
viewed as a kernel function. In Appendix \aga{ref} we show that for learning the gravity function
the NTK kernel for ReLU 
activation has superior learning guarantees than the Gaussian kernel. Our theory may enable a more detailed analysis
of popular models on tasks of interest.

==> old_version.tex <==
\begin{theorem}\label{thm:clusterfunctions}
The function $ f(x) = \sum_{j=1}^{K} \exp(- \alpha || x - c_j ||^2) f_j((x - c_j)/r )$ when evaluated on an input $c_j + r x$ has value $f_j(x) \pm \epsilon $. If each $f_j$ is a degree $p$ polynomail in variables $<\beta_i, x>$ with $l_1$ norm of the coefficient at most $1$ and $||\beta_i||_2 = 1$ for all $i$, then this combined function can be learned with $poly((k/\epsilon)^p)$ examples. We set $r=1/\alpha$. More generally the norm is $poly(k/\eps)$ times sum of the norms of $f_j(x - c_j)/r$. The error in the output at most $1/\alpha$
This automatically gives us lookup tables as long as the keys $c_i$ are well separated (without even needing scaling by $r$)
[[Compare this with other method where you use $log k$ prefix bits. There you get dependence $d^{\log k}$. Here you don't get that but instead you get increased norm due to scaling input of $f$ by $1/\alpha$]]
\end{theorem}


\begin{proof}
Assume all the cluster centers are a constant distance apart. Then the cluster indicator function can be written as
\[
I_j(x) = \exp(- \alpha || x - c_j ||^2),
\]
assuming $x$ and the centers are all on unit sphere, this is proportional to  $\exp( \alpha <x, c_j>) $. We need to choose $\alpha$ so that this is close to $1$ within the $j$-th cluster, and at most $\epsilon/k$ in other clusters. This is achieved by setting $\alpha = \Theta(\log(k/\epsilon))$. Note if $x$ is from a different cluster, then $||x - c_j||$ is at least some constant, and so the $I_j(x)$ is at most $\epsilon/k$. The contribution from $k$ such clusters would be at most $\epsilon$. If $|| x - c_j || < \epsilon/k$, then the value is at least $\exp(\log(k/\epsilon) (\epsilon/k)^2 ) \geq 1 - O(\epsilon/k)$. 

If $y = <x, c>$
\[
\tilde{I}_{j}(y) = \exp(\alpha y - 2) \Rightarrow \tilde{I}_{j}(1) = \exp(\alpha - 2) \leq e^{\alpha} = poly(k/\epsilon)
\]

Given $f_j$, suppose it is a polynomial of degree at most $p$ in variables $<\beta_i, x>$, and the $l_1$ norm of the coefficient vector of the polynomial is at most $1$, and the $l_2$ norm of all the $\beta_i$'s are $1$, then if we replace $x$ by $(x- c)/r$, we get a new polynomial in $<\beta_i, x>$ where the sum of the absolute value of the coefficients is at most $(2/r)^p = (k/\epsilon)^p$.
\end{proof}

% old Decision tree proof


For each indicator function $I_j(\mathbf{x})$, we have 
$I_{j}(\mathbf{x}) = \prod_{l=1}^{k_j} \left(a_{j_l} x_{j_l} + b_{j_l}\right)$, therefore, by Cor. 0.1 (Atish), it is learnable with $\sqrt{M_{I_j}} = k_j \prod_{l_j} \beta_l$, where $\beta_l = \sqrt{a_{l_j}^2 + b_{l_j}^2} = \sqrt{d/2}$. Note $k_j \leq h$, where $h$ is the depth of the decision tree. Then $\sqrt{M_{I_j}} \leq h (d/2)^{h/2}$.

Now for the product, by Cor. 1.1 (Atish), we have $\sqrt{M_{I_j f_j}} \leq \sqrt{M_{I_j}}  \tilde{f}_j(1) + \tilde{I}_{j}(1) \tilde{f}'_j (1) \leq h (d/2)^{h/2} \tilde{f}_j(1) + \tilde{I}_{j}(1) \tilde{f}'_j (1)$. Note here $\tilde{I}_{j}(1) = \prod_{l=1}^h \sqrt{d/2} = (d/2)^{h/2}$, so we get $\sqrt{M_{I_j f_j}} \leq (d/2)^{h/2} ( h \tilde{f}_j(1) + \tilde{f}'_j (1) )$.

For the sum, by the discussion after theorem 6.1 in the Arora paper, we have $\sqrt{M_f} \leq \sum_j \sqrt{M_{I_{j} f_j}} \leq (d/2)^{h/2} \sum_{j} ( h \tilde{f}_j(1) + \tilde{f}'_j (1) ) = (d/2)^{h/2} (C h + D)$, where $C$ and $D$ are constants that depends on the leaf functions $f_j$, $j = 1, 2, ..., B$.


\begin{theorem}
For constant depth, a generalized decision program with $k$ nodes can be represented by a polynomial of degree at most $\poly\log(k/\eps)$. The sample complexity is at most $d^{\poly\log(k/\eps)}$.


%The above generalized decision program can be represented as a poly of degree at most $\log(k/\eps)^h$. The overall complexity is $2^{polylog(k/\eps)}$ for constant $h$.
\end{theorem}

1. Object representation: combining fields into a single object, and accessing a certain field given an object. 
By packing the different fields in an object into orthogonal subspaces, we can get a sketched representation of the object. If the different fields are computed by functions representable by subtrees in the class C, then the entire The fields of the objects can be accessed by projection. 

1.5. Any analytic function. 

2. Function composition: If $f, g$ are representable then so is $f(g(x))$. Note that if $f$ takes multiple arguments then $g$ may return a tuple. 

3. Look up tables: Simple key, value look up is supported. 

4. SQL style predicated look up and aggregation is supported. Note: approximate max reduces to sum of appropriately scaled threshold indicators


Class C of supported functions: Each node is R*y where each entry is y is an analytic function of the child nodes. It may also be a decision node based on margin or by proximity to a collection of centers.

[[
Toy programming constructs:

1. We support simple object oriented functional constructs including:

Objects and Classes. Classes form a hierarchy of constant depth but unbounded width.

Classes can have fields which can be previously defined classes or atomic data types.

Base functions are : Any analytic function such as + , *, /, sin , cos.

switch statements on a variable (any function output). Note that subsumes table lookup

Each method is implemented as a functional program that is some analytic composition of previously defined functions.

Example program: Find average salary of a subset of people in a salary table.
Example program: Find average salary of people where person.address.city = input-city
This is more than a switch statement. This is  map followed by an aggregator (sum)

Is this like SQL? SQL 
]]
